An analysis of Universal Differential Equations for data-driven discovery of Ordinary Differential Equations

In the last decade, the scientific community has devolved its attention to the deployment of data-driven approaches in scientific research to provide accurate and reliable analysis of a plethora of phenomena. Most notably, Physics-informed Neural Networks and, more recently, Universal Differential Equations (UDEs) proved to be effective both in system integration and identification. However, there is a lack of an in-depth analysis of the proposed techniques. In this work, we make a contribution by testing the UDE framework in the context of Ordinary Differential Equations (ODEs) discovery. In our analysis, performed on two case studies, we highlight some of the issues arising when combining data-driven approaches and numerical solvers, and we investigate the importance of the data collection process. We believe that our analysis represents a significant contribution in investigating the capabilities and limitations of Physics-informed Machine Learning frameworks.

==> prob_descr.tex <==
To draw solid conclusion, we will answer these questions considering two different use cases:
%
    \begin{itemize}
        \item Predictions of the number of infected people during a pandemic.
        \item Estimation of the final voltage of a first-order Resistor-Capacitor (RC) circuit.
    \end{itemize}
%

% EPIDEMICS
\subsection{Compartmental Models}

In traditional predictive epidemiology the use of dynamic systems has been one of the basis of the discipline, which proved to be effective in modeling the spreading of infectious disease. 
Most notably, Compartimental Models (CM) provide a compact formulation of complex phenomena such as epidemics. 
The idea is to divide the population into categories, or compartments, which represent a specific state of the individuals w.r.t. to the disease. 
For instace, one of the simplest example of this approach, is the \textbf{SIR} model, namely \textbf{S}usceptible-\textbf{I}nfected-\textbf{R}ecovered. 
The transition to one compartment to the other is described by set of differential equations:
\begin{align*}
    \frac{dS}{dt} &= - \beta~\frac{S\cdot I}{N} \\ \nonumber
    \frac{dI}{dt} &= \beta~\frac{S\cdot I}{N} - \gamma~I \\ \nonumber
    \frac{dS}{dt} &= \gamma~I \nonumber
\end{align*}
, where $N$ represents the total amount of individuals in the population, $\gamma$ depends on the average recovery time of an infected subject, whereas $\beta$ is the number of contact needed per time steps to have a new infected in the susceptible population; the $R_0$ factor, or  \textit{basic reproductive number}, that is the number of infections generated by each infectious person, is obtained the quotient of the two parameters, $\frac{\beta}{\gamma}$. Figure \ref{fig:sir} shows a SIR simulation of one year.
%
\begin{figure}[h]
        \centering
             \includegraphics[width=0.5\textwidth]{images/sir.png}
                \caption{SIR curve generated with following initial conditions: $S_0=99\%$, $I_0=1\%$, $R_0=0\%$, $\gamma=\frac{1}{15}$, $\beta=0.3$}
    \label{fig:sir}
\end{figure}
%
The parameter $\beta$ in particular, is of high interest since it basically determines the spreading coefficient of the epidemic. 
This value is highly dependent on environmental factors (e.g., temperature, density of the population, contact rate) and, most importantly, interventions aimed at containing the spreading of the disease. 
In the scope of this paper, we will mainly focus on a specific type of internvetions, i.e., \textbf{Non-Pharmaceutical Intervetions} (NPIs), that are the policies tackling the disease from a political and logistical perspective (quarantines, masks) rather than a clinical one. \fixme{I would not put such an high emphasis on NPI since we use synthetic data.}
\\
\\
The UODE framework can be adapt to CM, in particular, we will focus on two application: 1) fitting an accurate parametrization of the SIR model and 2) estimating the impact of a set of NPIs in the spreading of the virus. 
\fixme{Shall we specify now that we will be concerned only with $\beta$? Or shall we stay general and than specify it in the results section? I believe it might be more general keeping it as it is, in the end the approach can be used with any number of parameters}
\fixed{Yes, I think we should provide a general outline of the method (UODE) and then only describe which parameters we will focus on.}
\\
\\
The first problem is focused on finding an accurate series of parameters compatible with the historical data relative to an outbreak. 
This can be achieved considering the parameters of the network itself as the weights of the universal approximator utilized at training process, namely a neural network. 
If we consider the initial formulation of UODE:
\[U_{\theta}(u, t) = \theta\]
, where $\theta$ coincides with the parametrization of the SIR model (e.g., $\beta$ and $\gamma$). 
\fixme{Same thing, shall I specify now the architecture of the network? ("srotolata"), or I keep it for the experimental part}
\fixme{We should probably describe in the method or background description the difference between the full unrolling and the decomposition of the dynamic system curve.}
\\
\\
The universal estimator used to approximate the differential system can depend on an arbitrary set of additional variables. 
This paves the way to the second application of UODE for epidemics forecasting. 
The prediction of the final model can be integrated with NPIs to estimated their effect on the outcome. 
In the scope of this paper, the universal approximator is tasked with predicting the parameter configuration of the dynamic system in time, therefore, the outcome of the model produces an estimate of the parameters in presence of a specific instance of the NPIs. Thus, the UODE formulation can be written as follows:
\[u' = f(u, t, U_{\theta}(u, t, X_t))\]
, where $X_t$ represents the NPIs instance at time $t$.

%
% RC CIRCUIT WITH CONSTANT VOLTAGE GENERATOR
\subsection{RC circuit with constant voltage generator}
\fixme{We have to find a consistent notation.}

A first-order RC circuit is an electric circuit with one resistor and one capacitor. The capacitor is the dynamic component and its behavior over time can be driven by a voltage or current generator. Here, we will consider a first-order RC circuit with a constant voltage generator.
%
    \begin{figure}[h]
        \centering
             \includegraphics[width=5cm]{images/rc-circuit.png}
                \caption[Schema of a first-order RC-circuit.]{Schema of a first-order RC-circuit.}
    \label{fig:seconda}
    \end{figure}
%
The analytical formula of the capacitor voltage is:
%
\begin{equation}
    v_c(t) = (v_c(0) - V_s) e ^ {(-t / \tau)} + V_s
    \label{eq:rcformula}
\end{equation}
%
and the differential equation that describes the capacitor voltage over time is:
%
    \begin{equation}
        \frac{dv_{C}(t)}{dt}=\frac{1}{\tau}(V_s - v_C(t))
     \label{eq:rcderivative}
    \end{equation}
%
where $v_C(t)$ is the capacitor voltage at time $t$, $V_s$ is the voltage provided by the generator and $\tau$ is the time constant which defines the circuit response.
RC circuits have characteristic charge/discharge behaviors, as shown in \cref{fig:rcchargedischarge}.
%
    \begin{figure}[h]
        \centering
            \includegraphics[width=0.35\textwidth]{images/rc-ramps.png}
                \caption[RC-circuit charge/discharge behaviors.]{RC-circuit charge/discharge behaviors.}
    \label{fig:rcchargedischarge}
    \end{figure}
%
Despite being simple, RC circuits are usually employed as a simplified schema for high-complexity systems \fixme{Put some citations.}

For this use case, we can suppose $\tau$ and/or $V_s$ unknown and apply the \uodeacronym{} formulation of \cref{eq:universalode} to approximate them, thus obtaining:
%
   %
    \begin{equation}
        u^{\prime}=\frac{1}{U_{\theta_1}(t)}(U_{\theta_2}(t) - u(t))
     \label{eq:uderc}
    \end{equation}
% 
Assuming to have measurements of the capacitor voltage at discrete timesteps $t$, we can rewrite \cref{eq:uodecostfunction} as:
%
    \begin{equation}
        C(U_{\theta_1}(t), U_{\theta_2}(t)) = \sum_{t}(V(t, U_{\theta_1}(t), U_{\theta_2}(t))-\hat{V}(t))^2 
    \end{equation}
%
where $V(t, U_{\theta_1}(t), U_{\theta_2}(t))$ are the predictions of the \uodeacronym{} and $\hat{V}(t)$ are the measured data.


==> src/background.tex <==
\subsection{Universal Differential Equations}
%Let consider a partial differential equation (PDE)

%    \begin{equation}
%        u(t, x) + \mathcal{N}[u(t, x); \lambda] = 0
 %       \label{eq:pinn}
 %   \end{equation}
%
%where $u(t, x)$ is the hidden solution with $x \in \Omega \subsetq \mathbb{R}^D$ the system state and $t \in \left[ 0, T \right]$ the time. $\mathcal{N} \left[\cdot \ ; \lambda \right]$ is a nonlinear operator parameterized by $\lambda$. 


%Neural Ordinary Differential Equations \cite{chen2018neural} provide a time-continuous definition of the neural networks' hidden state. The derivative of the hidden state is a function of the hidden state itself, namely $\frac{dh(t)}{dt} = f(h(t), t, \theta)$.

%\cite{rackauckas2020universal} are a generalization of Neural ODE where part of a differential equation is described by a universal approximator, such as a neural network. The formulation is general enough to allow the modeling of time-delayed, stochastic and partial differential equations:

The Universal Differential Equation (UDE) \cite{rackauckas2020universal} formulation relies on embedded universal approximators to 
model forced stochastic delay PDEs:

%
    \begin{equation}
        \mathcal{N} \left[ u(t), u(\alpha(t)), \text{W}(t), U_{\theta}(u, \beta(t)) \right] = 0
        \label{eq:UDE}
    \end{equation}
%
where $u(t)$ is the system state at time $t$,  $\alpha(t)$ is a delay function and $\text{W}(t)$ is the Wiener process. $\mathcal{N}$ is a nonlinear operator and $U_{\theta}$ is a universal approximator parameterized by $\theta$. 
The UDE framework is general enough to express other frameworks that combine physics knowledge and deep learning models. For example, by considering a one-dimensional UDE defined by a neural network, namely $u'= U_\theta (u(t), t)$, we retrieve Neural Ordinary Differential Equation frameworks \cite{chen2018neural,NEURIPS2019_42a6845a,NEURIPS2020_4a5876b4}.  and Physics-Informed Neural Networks (PINNs) \cite{raissi2019physics}. 

%Moreover, conversely to other Physics-Informed Neural Networks (PINNs) use partial differential equations in the cost functions of neural networks to incorporate prior scientific knowledge the UDE formalism is more suitable to integrate more recent and advanced numerical solvers, providing the basis for a library that supports a wide range of scientific application.

==> src/case_studies.tex <==
In this section, we report the results of our analysis performed on two case studies: 1) \textit{Predictive Epidemiology}, i.e., predicting the number of infected people during a pandemic; 2) \textit{RC circuit}, i.e.,  estimating the final voltage in a first-order resistor-capacitor circuit.
We start by describing the two case studies. Then, we describe the evaluation procedure and the experimental setup.
Finally, we illustrate the experiments focused on the research questions highlighted in Section \ref{sec:research_questions}, and we report the corresponding results.
%In particular, we are interested in 1) evaluating which training approach between \unrollmethod{} and \pairmethod{} is more suitable, 2) how the integration method accuracy impacts the estimation of the parameter, 3) whether the \uodeacronym{} can effectively reconstruct a functional dependence between a set of observables and the ODE parameters, 4) how the data collection process affects the approximation accuracy, and 5) whether \uodeacronym{} can learn a probability distribution associated with the ODE parameters.
%
%Despite being both defined by a system of ODEs, these models describe very different physical phenomena. Moreover, they have notable differences that make them worth of attention. In the SIR model, the state is a vector $\mathbf{u} \in \mathbb{R}^3$ and it is described by a set of $3$ equations that are non-linear in the susceptible and infected. On the other side, the state $\mathbf{u}$ of the RC circuit is a simple scalar and its dynamics are described by a single linear equation \msilv{Do you think that these comments are worth to be mentioned? If so, shall we put them when we introduce the two problems?}. Also, the two systems differ in the number of parameters to estimate. In the case of epidemics, one value regulates the amount of newly infected (i.e., $\beta$), while for the RC-circuit, the capacitor voltage depends on both the source and the time constant.

% CASE STUDY: PREDICTIVE EPIDEMIOLOGY
\subsubsection{Predictive Epidemiology}

Among the different compartmental models used to describe epidemics, we consider the well-known Susceptible-Infected-Recovered (SIR) model, where the disease spreads through the interaction between susceptible and infected populations.
The dynamics of a SIR model are described by the following set of differential equations:
%
\begin{align}
    \begin{split}
            \frac{dS}{dt} &= - \beta~\frac{S\cdot I}{N}, \\ 
        \frac{dI}{dt} &= \beta~\frac{S\cdot I}{N} - \gamma~I, \\ 
        \frac{dR}{dt} &= \gamma~I ,
    \end{split}
    \label{eq:sir}
\end{align}
%
where $S,I$, and $R$ refer to the number of susceptible, infected, and recovered individuals in the population. The population is fixed, so $N = S+I+R$. The parameter $\gamma \in [0,1]$ depends on the average recovery time of an infected subject, while $\beta \in [0,1]$ is the number of contacts needed per time steps to have a new infected in the susceptible population. $\beta$ determines the spreading coefficient of the epidemic and is strongly affected by different environmental factors (e.g.,  temperature, population density, contact rate, etc.). The introduction of public health measures that directly intervene on these environmental factors allows to contain the epidemic spreading.

We rely on the \uodeacronym{} framework (i) to perform system identification on a simulated SIR model, and (ii) to estimate the impact of \textit{Non-Pharmaceutical Interventions} (NPIs) on the epidemic spreading.
We define the state of the system at time $t$ as $\mathbf{u}_t = (S_t,I_t,R_t)$ and we formulate the Equations in \eqref{eq:sir} as


%\begin{equation}
%    \mathbf{u}'  = 	
%    \begin{bmatrix} 
	%f_1(\mathbf{u}_t, t, U_{\theta}(\mathbf{u}_t, t, X_t)) \\
	%f_2(\mathbf{u}_t, t, U_{\theta}(\mathbf{u}_t, t, X_t)) \\
	%f_3(\mathbf{u}_t, t, U_{\theta}(\mathbf{u}_t, t, X_t)) \\
	%%\end{bmatrix}

    %%\label{eq:sir_ude}
%\end{equation}

%
\begin{equation}
    \mathbf{u}' = f(\mathbf{u}_t, t, U_{\theta}(\mathbf{u}_t, t, X_t))
\end{equation}
%

where 
%$f$ is function of time and state and 
$X_t$ is the set of NPIs applied at time $t$. We approximate the  SIR model parameters $\alpha$ and $\gamma$ with a neural network $U_{\theta}(\mathbf{u}_t, t, X_t)$, where $\theta$ coincides with the SIR parameters $\alpha$ and $\gamma$. 

The cost function for this case study is defined as 
%
    \begin{equation}
        C_{\theta} = \sum_{i}(u_{\theta}(t_i)-\hat{y}_i)^2 
    \end{equation}
%
where $u_{\theta}(t_i)$ and $y_i$ are the current solution and the discrete-time measurements of the system state at time $t_i$, respectively.

% CASE STUDY: RC circuit
\subsubsection{RC Circuit}

We consider a first-order RC circuit with a constant voltage generator. The state evolution of the system is described by
%
\begin{equation}
    \frac{dV_{C}(t)}{dt}=\frac{1}{\tau}(V_s - V_C(t))
 \label{eq:rcderivative}
\end{equation}
%
where $V_C(t)$ is the capacitor voltage at time $t$, $V_s$ is the voltage provided by the generator, and $\tau$ is the time constant which defines the circuit response.

We use the \uodeacronym{} formulation to approximate  $\tau$ and $V_s$ by writing Equation \eqref{eq:rcderivative} as
%
   %
    \begin{equation}
        \mathbf{u}^{\prime}=\frac{1}{U_{\theta_1}(t)}(U_{\theta_2}(t) - \mathbf{u}(t))
     \label{eq:uderc}
    \end{equation}
% 
where $u_t$ is a short notation for $V_C(t)$, $U_{\theta_1}(t)$ and $U_{\theta_2}(t)$ are the neural networks approximating $\tau$ and $V_s$ respectively.

The cost function is defined as 
%
    \begin{equation}
        C_{\theta_1,\theta_2} = \sum_{i}(u_{\theta_1,\theta_2}(t_i)-y_i)^2 
    \end{equation}
%
where $u_{\theta_1,\theta_2}(t_i)$ and $y_i$ are the current solution and the discrete-time measurements of the capacitor voltage at time $t_i$, respectively.

%By assuming to have measurements of the capacitor voltage at discrete time steps $t$, we can rewrite the cost function \cref{eq:uodecostfunction} as

%where $u(t, U_{\theta_1}(t), U_{\theta_2}(t))$ are the predictions of the \uodeacronym{} and $\hat{u_t}$ are the measured data.



==> tables/batch_RC_stoch.tex <==
\begin{table*}
\centering
\caption{Da spostare in sezione stocastica. TODO: caption}
\label{table:batch_rc_stoch}
\vspace{2pt}
\addtolength{\tabcolsep}{4pt}
\small
\begin{tabular}{lcccc}
\toprule
%{} & \multicolumn{2}{c}{R2} & \multicolumn{2}{c}{GeDI-V1 \%} & \multicolumn{1}{c|}{Time} & \multicolumn{2}{c}{Accuracy} & \multicolumn{2}{c}{GeDI-V1 \%} & {Time} \\
{} & {$V_s$}  & {$\tau$}  & {$V_c(t)$} & {Time}\\
\midrule
     \pairmethod{}   & $0.13 \pm 0.094$  &  $0.38\pm 0.102 $  &  $0.02 \pm 0.010$  &  
     $1.44 \pm 0.26$ \\
    \unrollmethod{} &   $0.12 \pm 0.086$  & $0.38 \pm 0.098 $  & $0.03 \pm 0.012$  & $1.46 \pm 0.51$ \\
\bottomrule
\end{tabular}
\label{exp1stoch}
\end{table*}


==> tables/batch_SIR_stoch.tex <==
\begin{table*}
\centering
\caption{Da spostare in sezione stocastica. TODO: caption}
\label{table:batch_sir_stoch}
\vspace{2pt}
\addtolength{\tabcolsep}{4pt}
\small
\begin{tabular}{lccc}
\toprule
%{} & \multicolumn{2}{c}{R2} & \multicolumn{2}{c}{GeDI-V1 \%} & \multicolumn{1}{c|}{Time} & \multicolumn{2}{c}{Accuracy} & \multicolumn{2}{c}{GeDI-V1 \%} & {Time} \\
{} & {$\beta$}  & {$SIR(t)$}  & {Time}\\
\midrule
     \pairmethod{}  & $0.14 \pm 0.054$  & $0.27 \pm 0.18$  & $3.15 \pm 0.17$ \\
    \unrollmethod{} &  $0.067 \pm 0.051$ & $0.10 \pm 0.096$  & $25.38 \pm 5.47$ \\
\bottomrule
\end{tabular}
\label{exp1stoch}
\end{table*}

